Preventing Machine Learning Poisoning Attacks Using Authentication and Provenance

Recent research has successfully demonstrated new types of data poisoning attacks. To address this problem, some researchers have proposed both offline and online data poisoning detection defenses which employ machine learning algorithms to identify such attacks. In this work, we take a different approach to preventing data poisoning attacks which relies on cryptographically-based authentication and provenance to ensure the integrity of the data used to train a machine learning model. The same approach is also used to prevent software poisoning and model poisoning attacks. A software poisoning attack maliciously alters one or more software components used to train a model. Once the model has been trained it can also be protected against model poisoning attacks which seek to alter a model's predictions by modifying its underlying parameters or structure. Finally, an evaluation set or test set can also be protected to provide evidence if they have been modified by a second data poisoning attack. To achieve these goals, we propose VAMP which extends the previously proposed AMP system, that was designed to protect media objects such as images, video files or audio clips, to the machine learning setting. We first provide requirements for authentication and provenance for a secure machine learning system. Next, we demonstrate how VAMP's manifest meets these requirements to protect a machine learning system's datasets, software components, and models.

==> infer.tex <==
\section{Inference}
\label{sec:infer}
